TATA: Stance Detection via Topic-Agnostic and Topic-Aware Embeddings

Stance detection is important for understanding different attitudes and beliefs on the Internet. However, given that a passage's stance toward a given topic is often highly dependent on that topic, building a stance detection model that generalizes to unseen topics is difficult. In this work, we propose using contrastive learning as well as an unlabeled dataset of news articles that cover a variety of different topics to train topic-agnostic/TAG and topic-aware/TAW embeddings for use in downstream stance detection. Combining these embeddings in our full TATA model, we achieve state-of-the-art performance across several public stance detection datasets (0.771 $F_1$-score on the Zero-shot VAST dataset). We release our code and data at https://github.com/hanshanley/tata.

==> dead.tex <==
\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\label{tab:accents}
\end{table}
\section{Preamble}
\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\hline
\citep{ct1965} & \verb|\citep| & \verb|\cite| \\
\citealp{ct1965} & \verb|\citealp| & no equivalent \\
\citet{ct1965} & \verb|\citet| & \verb|\newcite| \\
\citeyearpar{ct1965} & \verb|\citeyearpar| & \verb|\shortcite| \\
\citeposs{ct1965} & \verb|\citeposs| & no equivalent \\
\citep[FFT;][]{ct1965} &  \verb|\citep[FFT;][]| & no equivalent\\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}



\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation: 
\begin{quote}
\tt\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}
\paragraph{Stance Detection:}



Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).


\subsection{References}

\nocite{Ando2005,borschinger-johnson-2011-particle,andrew2007scalable,rasooli-tetrault-2015,goodman-etal-2016-noise,harper-2014-learning}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{custom}
\end{verbatim}
\end{quote}
You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}
Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.

\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.


\begin{table*}

\centering

%\tiny

\fontsize{10pt}{8}

\selectfont

\setlength\tabcolsep{4pt}

\begin{tabular}{l|cccc|cccc|cccccc}

& \multicolumn{4}{c|}{\textbf{All VAST}}& \multicolumn{4}{c|}{\textbf{Zero-Shot VAST}} & \multicolumn{6}{c}{\textbf{SemEval2016t6}}  \\ \midrule

& Pro .& Con. & Neutral & All &  Pro . & Con. & Neutral &  All & DT& LA &HC  &FM &CC & AA\\ \midrule
TESTED & -  & - & - & 57.47 - & - & - & - & 54.33 & - & - & -\\
JointCL & 64.9 & 63.2 & 88.9 & 72.3  \\
TGA Net & 55.4 & 58.5 & 85.8 & 66.6 \\
CKE-Net & 61.2 & 61.2 & 88.0 & 70.2   \\
PT-HCL  & 61.7 & 63.5 & 89.6 & 71.6 &  \\

BERT & 0.63 &0.60 &0.89 &0.71 &0.65 & 0.63 & 0.85 &0.71 &0.47 & 0.66 & 0.70 & 0.63 & 0.82 & 0.73  \\
RoBERTa&0.68 & 0.64 & 0.90 & 0.74 & 0.64 & 0.61 & 0.85 & 0.70& 0.62 & 0.64 & 0.75 & 0.67 & 0.78 & 0.71 \\
DeBERTa & 0.70 &0.66 & 0.90 & 0.76 & 0.68 & 0.61 & 0.86 & 0.72& 0.57 & 0.69 & 0.72 & 0.71 & 0.79 & 0.74   \\
Topic-Agn./TAG& 0.72 &0.71 & 0.90 &0.78 & 0.69 & 0.70 & 0.87 & 0.75 & 0.56 & 0.70 & 0.65 & 0.64 & 0.77 & 0.69  \\
Topic-Aw./TAW & 0.70 & 0.70 & 0.90 & 0.77 & 0.67 & 0.69 & 0.87 & 0.75 &0.65 &0.74 & 0.72 & 0.72 & 0.82 & 0.79  \\
TATA &  0.66 & 0.67 & 0.88  \\

%0.452/1.0/0.292

\end{tabular}

\caption{\label{tab:benchmark} F1-scores of models on various benchmarks. We bold the highest/best score in each column. As seen our full TATa model performs the best across various benchmarks.}
\vspace{-10pt}
\end{table*}


\begin{table}

\centering

%\tiny

%\fontsize{10pt}{8}
\small
\selectfont

%\setlength\tabcolsep{4pt}

\begin{tabular}{l|cccc|}

& \multicolumn{4}{c|}{\textbf{Zero-Shot VAST}}  \\ \midrule

& Pro .& Con. & Neutral & All  \\ \midrule
TESTED & -  & - & - & 54.33 \\
JointCL & 64.9 & 63.2 & 88.9 & 72.3 \\
TGA Net & 55.4 & 58.5 & 85.8 & 66.6 \\
CKE-Net & 61.2 & 61.2 & 88.0 & 70.2   \\
PT-HCL  & 61.7 & 63.5 & 89.6 & 71.6   \\ \midrule
BERT & 0.63 &0.60 &0.89 &0.71 \\
RoBERTa&0.68 & 0.64 & 0.90 & 0.74  \\
DeBERTa & 0.70 &0.66 & 0.90 & 0.76  \\
Topic-Agn./TAG& 0.72 &0.71 & 0.90 &0.78  \\
Topic-Aw./TAW & 0.70 & 0.70 &\\
TATA &  0.66 & 0.67 & 0.88  \\

%0.452/1.0/0.292

\end{tabular}

\caption{\label{tab:benchmark} F1-scores of models on the Zero-Shot Vast dataset. We bold the highest/best score in each column. As seen our full TATa model performs on each label within VAST.}
\vspace{-10pt}
\end{table}



\begin{table}
\centering
\selectfont
\small
\begin{tabular}{l|rrrrr} \toprule
Model &Qte &Sarc &  Imp &mlS &  mlT \\\midrule
TGA-Net & 0.661& 0.637 & 0.623& 0.547 &0.624 \\ \midrule
BERT  & 0.705 & 0.691& 0.608 & 0.555 & 0.639 \\
RoBERTa & 0.686 & 0.717 & 0.637 & 0.570 & 0.664 \\
DeBERTa & 0.698 & 0.733 &  0.663& 0.563 & 0.674 \\
TAG & \textbf{0.720} & 0.712 & 0.672 &0.614 &0.685  \\ % Good  
TAW & 0.711 & \textbf{0.745} & 0.670& 0.579 & 0.673  \\ %Good
TATA & 0.711 & 0.731 & \textbf{0.703} &\textbf{0.620} & \textbf{0.705} \\
\bottomrule
\end{tabular}

\vspace{-5pt}
\caption{\label{tab:dataset} Accuracies on various phenomena with the VAST test set. We give accuracies here to directly compare our results against~\citet{allaway2020zero}. } 
\vspace{-15pt}
\end{table}


DeBERTa & 0.682 &0.682 & 0.907 & 0.757&   \\
TAG& 0.648 &\textbf{0.709} & 0.891 &0.749 &   \\ 
TAW & 0.702 & 0.673& 0.902 & 0.759  \\ 
TATA &  \textbf{0.723} & 0.685 &\textbf{0.908} &\textbf{0.777}  \\ \midrule
%BERT & 0.687 & 0.554 & 0.890 & 0.710 & 0.668 &  0.549 & 0.843 & 0.687  \\
%RoBERTa  & 0.675 & 0.685 & 0.902 & 0.754 & 0.659 & 0.638 & 0.847 & 0.718 \\
%RoBERTa&0.709 & 0.636 & 0.895 & 0.746 & \\


\begin{table*}

\centering


\fontsize{8pt}{10}

\selectfont

\setlength\tabcolsep{6pt}

\begin{tabular}{l|cccccc|r}

&\multicolumn{6}{c}{\textbf{Few-Shot SemEval2016t6}} \\ \midrule
& DT& LA &HC  &FM &CC & A &Avg\\ \midrule
DeBERTa  &0.540 & 0.671 & \textbf{0.759} & \textbf{0.722} & 0.443 & 0.735 & 0.645  \\
TAG &  0.453 & 0.634 & 0.679& 0.634 & 0.445 & 0.472  & 0.552 \\ 
TAW & 0.589 &\textbf{0.678} & 0.655 & 0.680 & \textbf{0.656} & \textbf{0.748} & 0.668  \\ 
TATA & \textbf{0.636} & 0.659& 0.696 & 0.702 & 0.636 & 0.690 & \textbf{0.673} \\ 

%0.452/1.0/0.292

\end{tabular}

\caption{\label{tab:benchmark} Macro Avg of the ``Favor'' and ``Against'' classes for the SemEval dataset for our set of trained models. We bold the highest/best score in each column. As seen our full TATa model performs the best across various benchmarks. Our TATA model performs the best on average. }
\vspace{-10pt}
\end{table*}

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{emnlp2023-latex/figures/model_new.drawio.pdf}
\caption{Topic-Agnostic  and Topic-Aware (TATA) Network. $v_t$ is the topic embedding, $v_d$ is the document embedding, $v_{tag}$ is the  topic-agnostic encoding, and $v_{taw}$ is the topic-aware encoding  }
\vspace{-10pt}
\label{figure:topic-model}
\end{figure}



\begin{table*}

\centering


\fontsize{8pt}{10}

\selectfont

\setlength\tabcolsep{6pt}

\begin{tabular}{l|cccccc|r}
%%% FIX AVERAGES
&\multicolumn{6}{c}{\textbf{Few-Shot SemEval2016t6}} \\ \midrule
& DT& LA &HC  &FM &CC & A &Avg\\ \midrule
DeBERTa  &0.540 & 0.671 & \textbf{0.759} & \textbf{0.722} & 0.443 & 0.735 & 0.645  \\
TAG &  0.480 & 0.618 & 0.646& 0.642 & 0.403 & 0.506 & 0.509 \\ 
TAW & 0.589 &\textbf{0.678} & 0.655 & 0.680 & \textbf{0.656} & \textbf{0.748} & 0.668  \\ 
TATA & \textbf{0.636} & 0.659& 0.696 & 0.702 & 0.636 & 0.690 & \textbf{0.673} \\  % Todo 

%0.452/1.0/0.292

\end{tabular}

\caption{\label{tab:benchmark} Macro Avg of the ``Favor'' and ``Against'' classes for the SemEval dataset for our set of trained models. We bold the highest/best score in each column. As seen our full TATa model performs the best across various benchmarks. Our TATA model performs the best on average. }
\vspace{-10pt}
\end{table*}


\begin{table}
\centering
\selectfont
\small
\begin{tabular}{l|rrrr} \toprule
Dataset &Pro &Con &  Neutral & Total \\\midrule
vast &944  &1018  &1044 &  3,006\\
argmin & 4,944 & 6,195& 14,353 & 25,492\\
iac1 & 18,028 & 13,485 & 852 &  32,365 \\
ibmcs & 1,325 & 1,069 & 0 & 2,394  \\
poldeb & 3,964 & 3,170 &  0 & 7,143\\
semeval2016t6 & 1,057&  2,110 & 996 & 4,163\\
\bottomrule
\end{tabular}

\vspace{-5pt}
\caption{\label{tab:dataset}Number of examples per test dataset considered. Given that we train our models using only the VAST dataset, we benchmark our approach on \emph{all} examples present within the remaining datasets.} 
\vspace{-10pt}
\end{table}


\begin{table}

\centering


\fontsize{8pt}{10}

\selectfont

\setlength\tabcolsep{3pt}

\begin{tabular}{l|cccccc|r}
%%% FIX AVERAGES
&\multicolumn{6}{c}{\textbf{Few-Shot SemEval2016t6}} \\ \midrule
& DT& LA &HC  &FM &CC & A &Avg\\ \midrule
DeBERTa  &0.540 & 0.634 & \textbf{0.759} & \textbf{0.722} & 0.443 & 0.735 & 0.645  \\
TAG &  0.480 & 0.618 & 0.646& 0.642 & 0.403 & 0.506 & 0.509 \\ 
TAW & 0.589 &\textbf{0.678} & 0.670  & 0.680 & \textbf{0.656} & \textbf{0.748} & 0.668  \\ 
TATA & \textbf{0.626} & 0.445& 0.702 & 0.702 & 0.636 & 0.690 & \textbf{0.673} \\  % Todo 

%0.452/1.0/0.292
%Deberta DT, LA
%TAW, Hillary
%TATA DT,

\end{tabular}

\caption{\label{tab:sem16-results} Macro Avg of the ``Favor'' and ``Against'' classes for the SemEval dataset for our set of trained models. We bold the highest/best score in each column. As seen our full TATa model performs the best across various benchmarks. Our TATA model performs the best on average. }
\end{table}


\begin{figure*}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=0.95\linewidth]{emnlp2023-latex/figures/without_training_tsne.pdf}
  \caption{Before Training}
\label{fig:qanon-sub3}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=0.95\linewidth]{emnlp2023-latex/figures/one_epoch_training_tsne.pdf}
    \caption{1 Epoch}
  \label{fig:nine11-sub3}

\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=0.95\linewidth]{emnlp2023-latex/figures/two_epoch_training_tsne.pdf}
    \caption{2 Epochs}
  \label{fig:nine11-sub3}
\end{subfigure}

\caption{\textbf{t-SNE of VAST Dev Dataset at various steps During Contrastive Learning}-- As we train the Topic-Agnostic/TAG layer of our model on our augmented VAST training set, while not separating perfectly (illustrating the need for additional features)  clear ``Against'', ``Pro'', and ``Neutral'' clusters appear in the TSNE of the embeddings of the VAST Dev Dataset. As confirmed elsewhere~\cite{allaway2020zero,liang2022zero}, the ``Neutral'' category of examples is the most differentiable from ``Pro'' and ``Against.''  }
  \label{figure:conspiracies-to-different-types}
  \vspace{-15pt}
\end{figure*}

\begin{figure}
\noindent\fcolorbox{black}{white}{%

\begin{minipage}{.47\textwidth}
\scriptsize

\textbf{Original Text:}Regulation of corporations has been subverted by corporations. States that incorporate corporations are not equipped to regulate corporations that are rich enough to influence elections, are rich enough to muster a legal team that can bankrupt the state. Money from corporations and their principals cannot be permitted in the political process if democracy is to survive." \\

\textbf{Paraphrase Text:} The corporations have subverted the regulation of corporations. A state, which is not sufficiently rich to influence elections, is not sufficiently rich to muster a legal team that can bankrupt the state. If democracy is to survive, the money of corporations and their principals must be excluded from the political process.
\end{minipage}}
\caption{\label{fig:paraphrase-example} Example paraphrase of a text from our dataset.} 
\end{figure}
\begin{table}
\centering
\selectfont
\small
\begin{tabular}{l|rrr} \toprule
Target & Favor & Against & Neutral \\ \midrule
Donald Trump & 148  &200 & 260 \\
Hillary Clinton & 163 & 565 & 256 \\
Feminist Movement & 268 & 511 & 170 \\
Legalization of Marijuana & 167 & 544 & 222 \\
Atheism & 124 & 464 & 145 \\
Climate Change &335 & 26 & 203 \\
\bottomrule
\end{tabular}

\vspace{-5pt}
\caption{\label{tab:dataset-sem} Statistics for the \texttt{SEM16} dataset. } 
%\vspace{-15pt}
\end{table}
\noindent
